A Kernel Test for Three-Variable Interactions

We introduce kernel nonparametric tests for Lancaster three-variable interaction and for total independence, using embeddings of signed measures into a reproducing kernel Hilbert space. The resulting test statistics are straightforward to compute, and are used in powerful interaction tests, which are consistent against all alternatives for a large family of reproducing kernels. We show the Lancaster test to be sensitive to cases where two independent causes individually have weak influence on a third dependent variable, but their combined effect has a strong influence. This makes the Lancaster test especially suited to finding structure in directed graphical models, where it outperforms competing nonparametric tests in detecting such V-structures.

==> FactorA.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{016}[bc][bc]{\matlabtextA Null acceptance rate (Type II error)}%
\psfrag{017}[bc][bc]{\matlabtextA V-structure discovery: Dataset A}%
\psfrag{018}[tc][tc]{\matlabtextA Dimension}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{7}{7}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $1$}%
\psfrag{001}[ct][ct]{\matlabtextB $3$}%
\psfrag{002}[ct][ct]{\matlabtextB $5$}%
\psfrag{003}[ct][ct]{\matlabtextB $7$}%
\psfrag{004}[ct][ct]{\matlabtextB $9$}%
\psfrag{005}[ct][ct]{\matlabtextB $11$}%
\psfrag{006}[ct][ct]{\matlabtextB $13$}%
\psfrag{007}[ct][ct]{\matlabtextB $15$}%
\psfrag{008}[ct][ct]{\matlabtextB $17$}%
\psfrag{009}[ct][ct]{\matlabtextB $19$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rc]{\matlabtextB $0$}%
\psfrag{011}[rc][rc]{\matlabtextB $0.2$}%
\psfrag{012}[rc][rc]{\matlabtextB $0.4$}%
\psfrag{013}[rc][rc]{\matlabtextB $0.6$}%
\psfrag{014}[rc][rc]{\matlabtextB $0.8$}%
\psfrag{015}[rc][rc]{\matlabtextB $1$}%
%
%% </ytick>

==> FactorB.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{6}{6}\selectfont\strut}%
\psfrag{016}[cl][cl]{\matlabtextA CI: $X\!\perp\!\!\!\perp\!Y|Z$}%
\psfrag{017}[cl][cl]{\matlabtextA $\Delta_L$: Factor}%
\psfrag{018}[cl][cl]{\matlabtextA 2var: Factor}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{019}[bc][bc]{\matlabtextB V-structure discovery: Dataset B}%
\psfrag{020}[tc][tc]{\matlabtextB Dimension}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{7}{7}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $1$}%
\psfrag{001}[ct][ct]{\matlabtextC $3$}%
\psfrag{002}[ct][ct]{\matlabtextC $5$}%
\psfrag{003}[ct][ct]{\matlabtextC $7$}%
\psfrag{004}[ct][ct]{\matlabtextC $9$}%
\psfrag{005}[ct][ct]{\matlabtextC $11$}%
\psfrag{006}[ct][ct]{\matlabtextC $13$}%
\psfrag{007}[ct][ct]{\matlabtextC $15$}%
\psfrag{008}[ct][ct]{\matlabtextC $17$}%
\psfrag{009}[ct][ct]{\matlabtextC $19$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rc]{\matlabtextC $0$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.2$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.6$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.8$}%
\psfrag{015}[rc][rc]{\matlabtextC $1$}%
%
%% </ytick>

==> MarginalA.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{016}[bc][bc]{\matlabtextA Null acceptance rate (Type II error)}%
\psfrag{017}[bc][bc]{\matlabtextA Marginal independence tests: Dataset A}%
\psfrag{018}[tc][tc]{\matlabtextA Dimension}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{7}{7}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $1$}%
\psfrag{001}[ct][ct]{\matlabtextB $3$}%
\psfrag{002}[ct][ct]{\matlabtextB $5$}%
\psfrag{003}[ct][ct]{\matlabtextB $7$}%
\psfrag{004}[ct][ct]{\matlabtextB $9$}%
\psfrag{005}[ct][ct]{\matlabtextB $11$}%
\psfrag{006}[ct][ct]{\matlabtextB $13$}%
\psfrag{007}[ct][ct]{\matlabtextB $15$}%
\psfrag{008}[ct][ct]{\matlabtextB $17$}%
\psfrag{009}[ct][ct]{\matlabtextB $19$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rc]{\matlabtextB $0$}%
\psfrag{011}[rc][rc]{\matlabtextB $0.2$}%
\psfrag{012}[rc][rc]{\matlabtextB $0.4$}%
\psfrag{013}[rc][rc]{\matlabtextB $0.6$}%
\psfrag{014}[rc][rc]{\matlabtextB $0.8$}%
\psfrag{015}[rc][rc]{\matlabtextB $1$}%
%
%% </ytick>

==> MarginalB.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{6}{6}\selectfont\strut}%
\psfrag{016}[cl][cl]{\matlabtextA $\Delta_L$: $(X,Y)\!\perp\!\!\!\perp\!Z$}%
\psfrag{017}[cl][cl]{\matlabtextA 2var: $(X,Y)\!\perp\!\!\!\perp\!Z$}%
\psfrag{018}[cl][cl]{\matlabtextA 2var: $X\!\perp\!\!\!\perp\!Z$}%
\psfrag{019}[cl][cl]{\matlabtextA 2var: $X\!\perp\!\!\!\perp\!Y$}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{020}[bc][bc]{\matlabtextB Marginal independence tests: Dataset B}%
\psfrag{021}[tc][tc]{\matlabtextB Dimension}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{7}{7}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $1$}%
\psfrag{001}[ct][ct]{\matlabtextC $3$}%
\psfrag{002}[ct][ct]{\matlabtextC $5$}%
\psfrag{003}[ct][ct]{\matlabtextC $7$}%
\psfrag{004}[ct][ct]{\matlabtextC $9$}%
\psfrag{005}[ct][ct]{\matlabtextC $11$}%
\psfrag{006}[ct][ct]{\matlabtextC $13$}%
\psfrag{007}[ct][ct]{\matlabtextC $15$}%
\psfrag{008}[ct][ct]{\matlabtextC $17$}%
\psfrag{009}[ct][ct]{\matlabtextC $19$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rc]{\matlabtextC $0$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.2$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.6$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.8$}%
\psfrag{015}[rc][rc]{\matlabtextC $1$}%
%
%% </ytick>

==> TotalA.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{016}[bc][bc]{\matlabtextA Null acceptance rate (Type II error)}%
\psfrag{017}[bc][bc]{\matlabtextA Total independence test: Dataset A}%
\psfrag{018}[tc][tc]{\matlabtextA Dimension}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{7}{7}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $1$}%
\psfrag{001}[ct][ct]{\matlabtextB $3$}%
\psfrag{002}[ct][ct]{\matlabtextB $5$}%
\psfrag{003}[ct][ct]{\matlabtextB $7$}%
\psfrag{004}[ct][ct]{\matlabtextB $9$}%
\psfrag{005}[ct][ct]{\matlabtextB $11$}%
\psfrag{006}[ct][ct]{\matlabtextB $13$}%
\psfrag{007}[ct][ct]{\matlabtextB $15$}%
\psfrag{008}[ct][ct]{\matlabtextB $17$}%
\psfrag{009}[ct][ct]{\matlabtextB $19$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rc]{\matlabtextB $0$}%
\psfrag{011}[rc][rc]{\matlabtextB $0.2$}%
\psfrag{012}[rc][rc]{\matlabtextB $0.4$}%
\psfrag{013}[rc][rc]{\matlabtextB $0.6$}%
\psfrag{014}[rc][rc]{\matlabtextB $0.8$}%
\psfrag{015}[rc][rc]{\matlabtextB $1$}%
%
%% </ytick>

==> TotalB.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{6}{6}\selectfont\strut}%
\psfrag{016}[cl][cl]{\matlabtextA $\Delta_{tot}$: total indep.}%
\psfrag{017}[cl][cl]{\matlabtextA $\Delta_L$: total indep.}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{018}[bc][bc]{\matlabtextB Total independence test: Dataset B}%
\psfrag{019}[tc][tc]{\matlabtextB Dimension}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{7}{7}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $1$}%
\psfrag{001}[ct][ct]{\matlabtextC $3$}%
\psfrag{002}[ct][ct]{\matlabtextC $5$}%
\psfrag{003}[ct][ct]{\matlabtextC $7$}%
\psfrag{004}[ct][ct]{\matlabtextC $9$}%
\psfrag{005}[ct][ct]{\matlabtextC $11$}%
\psfrag{006}[ct][ct]{\matlabtextC $13$}%
\psfrag{007}[ct][ct]{\matlabtextC $15$}%
\psfrag{008}[ct][ct]{\matlabtextC $17$}%
\psfrag{009}[ct][ct]{\matlabtextC $19$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rc]{\matlabtextC $0$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.2$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.6$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.8$}%
\psfrag{015}[rc][rc]{\matlabtextC $1$}%
%
%% </ytick>
